On Correcting Inputs: Inverse Optimization for Online Structured Prediction

Algorithm designers typically assume that the input data is correct, and then proceed to find "optimal" or "sub-optimal" solutions using this input data. However this assumption of correct data does not always hold in practice, especially in the context of online learning systems where the objective is to learn appropriate feature weights given some training samples. Such scenarios necessitate the study of inverse optimization problems where one is given an input instance as well as a desired output and the task is to adjust the input data so that the given output is indeed optimal. Motivated by learning structured prediction models, in this paper we consider inverse optimization with a margin, i.e., we require the given output to be better than all other feasible outputs by a desired margin. We consider such inverse optimization problems for maximum weight matroid basis, matroid intersection, perfect matchings, minimum cost maximum flows, and shortest paths and derive the first known results for such problems with a non-zero margin. The effectiveness of these algorithmic approaches to online learning for structured prediction is also discussed.

==> matroid-intersection-proof.tex <==
\section{Matroid Intersection - Omitted Proof}
\label{sec:missingproofs}

We now prove the following $\delta$-optimality condition for the matroid intersection problem. 
Let $G(B,B')$ denote the subgraph induced on the $G$ by the vertex sets $B \setminus B'$ and $B' \setminus B$. Further, let $G_1 = (V,A_1)$ and $G_2 = (V,A_2)$ where $A_1$ and $A_2$ are as defined in the definition of the exchange graph $G$.
We'll refer to two well-known lemmas (for e.g. see Schrijver \cite{schrijver2003}) regarding the relationship between bases of a matroid and matchings in the exchange graph.
\begin{lemma}
\label{lemma:perfect-matching}
  If $B'$ is a basis of  matroid \M{1} $[\M{2}]$, then $G_1(B,B')[G_2(B,B')]$ contains a perfect matching.
\end{lemma}

\begin{lemma}
\label{lemma:unique-perfect-matching}
  For $B' \subseteq S$, if $G_1(B,B') [G_2(B,B')]$ has a \emph{unique} perfect matching, then $B'$ is a basis of \M{1} $[\M{2}]$.
\end{lemma}

Observe the asymmetry in the above two lemmas. The requirement of a \emph{unique} perfect matching causes the following proof to be a bit more involved.

\begin{lemma}[Matroid Intersection $\delta$-optimality condition]
\label{lemma:optimality-condition2}
The given common basis $B$ is $\delta$-optimal if and only if the exchange graph G contains no cycles having length less than $\delta$.  
\end{lemma}

\begin{proof}
{\bf Sufficiency:}  
This is the easy direction.

Let $B'$ be any common basis other than $B$. Look at the subgraph $G(B,B')$. Applying Lemma \ref{lemma:perfect-matching}, we know that $G(B,B')$ has two perfect matchings (one each in $G_1(B,B')$ and $G_2(B,B')$). Union of these two perfect matchings yields a collection of cycles $\mathcal{C}$. Further, by construction, by traversing these cycles, one can transform $B \rightarrow B'$. Hence, we have
\[w(B') = w(B) - \sum_{C \in \mathcal{C}}l(C)\]
Therefore, since we have $l(C) > \delta$ for all cycles, we are guaranteed that $w(B') < w(B) - \delta$ as desired.

{\bf Necessity:}
Ideally, we would like to say that every cycle in $G$ leads to a swapping such that the set so obtained is also independent in both the matroids. This would immediately imply that a cycle of small length would lead to a common basis $B'$ which is not much smaller than $B$.

However, the presence of a cycle simply implies the presence of a perfect matching (one in each direction) which may not be \emph{unique}. For example, Figure \ref{fig:original} shows an instance of an arborescence problem (left), and the associated exchange graph (right). Here $G$ contains a cycle a-x-b-y-a which leads to a new set ${x,y,c}$ which is not an arborescence. 

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.5\textwidth]{no_unique_matching.pdf}
  \caption{Instance showing every cycle in $G$ need not lead to a common basis}
  \label{fig:original}
\end{figure}

In the previous example, observe that if the cycle a-x-b-y-a were to have small weight, that would imply that at least one of a-y-a or b-x-b cycles too has small weight both of which lead to a feasible solution. This observation motivates us to look at the \emph{smallest} cycle of weight less than $\delta$ and hope that it does induce an \emph{unique} perfect matching.

Suppose that the graph has a cycle having weight less than $\delta$. Let $C$ be the smallest (in terms of number of arcs) such cycle. Look at the graph induced by the vertex set of the cycle. We claim that this induced subgraph has a unique perfect matching (one in each direction). Here we prove the claim for one direction. $C$ being an even cycle trivially contains a perfect matching $M$ from $B$-side to $S \setminus B$-side. Suppose there exists another perfect matching $M'$. For every edge $(x,y)$ in $M' \setminus M$, the edge along with the path between $y$ and $x$ in $C$ cause a cycle. Further, each such cycle is smaller (number of edges) than $C$. 

Let $\bar{M}$ denote the matching $M$ with edge directions reversed. The union of $M'$ and $\bar{M}$ now forms a collection of cycles. Consider any such cycle $D$. WLOG let the cycle be $(x_0, y_0, x_1, y_1, \ldots, x_k, y_k, x_0)$ such that the $(x_{i+1}, y_i)$ are edges in $M$ (i.e. $(y_i, x_{i+1}) \in \bar{M}$) and $(x_i,y_i) \in M'$. [All arithmetic is modulo $k+1$]. We'll now be interested in the length of the path between these vertices in the original cycle $C$. Let $C_i$ denote the cycle formed by the edge $(x_i,y_i)$ and the path between $y_i$ and $x_i$ in $C$. We have, 
\[l(C_i) = l(C) - l(\text{Path from $x_i$ to $y_i$ in $C$}) + l((x_i,y_i))\]
Since $(x_i, y_{i-1}) \in M$, 
\[l(\text{Path from $x_i$ to $y_i$ in $C$}) = l((x_i,y_{i-1})) + l(\text{Path from $y_{i-1}$ to $y_i$ in $C$})\]
Further since by construction $l((x,y_i)) = l((x,y_j)) ( = \pm w(x))$, we have
\[l(C_i) = l(C) - l(\text{Path from $y_{i-1}$ to $y_i$ in $C$})\]
Let $P_{i-1 \rightarrow i}$ denote this path. Summing over all $(x_i,y_i)$ edges in $D$, we get
\begin{align*}
  \sum_{i=0}^k l(C_i) &= k l(C) - (l(P_{k \rightarrow 0}) + l(P_{0 \rightarrow 1}) + \ldots + l(P_{k-1 \rightarrow k})) \\
  &= k l(C) - k' l(C) \\
\intertext{ $\uparrow$ Since we start from $y_k$, go around the $C$ and reach $y_k$ back}
  &= k'' l(C)\\
  &< k'' \delta
\intertext{The sum of $k$ weights is less than $k'' \delta$ with $k'' < k$, which implies}
\exists &C_i, \text{such that } l(C_i) < \delta
\end{align*}

But this is a contradiction since $C$ was the smallest cycle having weight less than $\delta$. Hence, the perfect matching $M$ is unique.

Similarly, the perfect matching induced by $C$ in the other direction too is unique. Applying Lemma \ref{lemma:unique-perfect-matching} successively on both sides, we know that $B'$ obtained by exchanging as per $C$ is a common basis for both matroids. Further, we have
\begin{align*}
  w(B') = w(B) - l(C) \\
  w(B') > w(B) - \delta
\end{align*}

Hence we have proved that if $G$ has a cycle with small weight, then $B$ is not $\delta$-optimal, thus proving the necessity of the claim.
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

